Can LLMs Solve longer Math Word Problems Better?

Math Word Problems (MWPs) play a vital role in assessing the capabilities of Large Language Models (LLMs), yet current research primarily focuses on questions with concise contexts. The impact of longer contexts on mathematical reasoning remains under-explored. This study pioneers the investigation of Context Length Generalizability (CoLeG), which refers to the ability of LLMs to solve MWPs with extended narratives. We introduce Extended Grade-School Math (E-GSM), a collection of MWPs featuring lengthy narratives, and propose two novel metrics to evaluate the efficacy and resilience of LLMs in tackling these problems. Our analysis of existing zero-shot prompting techniques with proprietary LLMs along with open-source LLMs reveals a general deficiency in CoLeG. To alleviate these issues, we propose tailored approaches for different categories of LLMs. For proprietary LLMs, we introduce a new instructional prompt designed to mitigate the impact of long contexts. For open-source LLMs, we develop a novel auxiliary task for fine-tuning to enhance CoLeG. Our comprehensive results demonstrate the effectiveness of our proposed methods, showing improved performance on E-GSM. Additionally, we conduct an in-depth analysis to differentiate the effects of semantic understanding and reasoning efficacy, showing that our methods improves the latter. We also establish the generalizability of our methods across several other MWP benchmarks. Our findings highlight the limitations of current LLMs and offer practical solutions correspondingly, paving the way for further exploration of model generalizability and training methodologies.

==> Chapters/conclusion.tex <==
\section{Conclusion}

Our study explores the impact of extended narrative contexts on LLMs' ability to solve MWPs, i.e. {\property}.
We introduce a groundbreaking dataset, {\benchmark}, designed to test {\property} of LLMs, along with two metrics to evaluate the efficacy and resilience of LLMs in this setting. 
Our investigation highlights a notable {\property} deficiency in existing zero-shot prompting techniques and open-source LLMs. 
The instructional prompting method and the novel SFT dataset we present not only significantly strengthen {\property} but also show promise in improving performance on traditional MWP datasets such as GSM8K. 
By illuminating a previously underexplored aspect of LLMs' reasoning capabilities and offering practical solutions to improve it, our work carves out new pathways for using LLMs in complex problem-solving and sets the stage for future research on model generalizability and advanced training paradigms.


==> Chapters/experiments.tex <==
\section{Results and Analysis}


\subsection{RQ1: Prompting Results}\label{sec: rslt-prompting}

\begin{table*}[ht]
\centering
\footnotesize
\begin{tabular}{ccccc}
\toprule
\thead{Large Language Models} & \thead{CoLeG-E} & \thead{CoLeG-R} & \thead{$\text{Acc}_0$} & \thead{$\text{Acc}_4$} \\
\midrule
\multicolumn{5}{c}{claude-3-opus-20240229} \\
\midrule
Plan-and-Solve & 74.30 & 83.56 & 95.45 & 79.76 \\
\rowcolor{gray!25} + Prompt & 77.63 (+3.34) & 86.04 (+2.48) & 95.60 (+0.15) & 82.26 (+2.50) \\
Plan-and-Solve+ & 74.53 & 83.77 & 95.30 & 79.83 \\
\rowcolor{gray!25} + Prompt & 77.18 (+2.65) & 84.90 (+1.13) & 95.91 (+0.61) & 81.43 (+1.59) \\
Zero-Shot CoT & 73.46 & 85.17 & 94.09 & 80.14 \\
\rowcolor{gray!25} + Prompt & 76.88 (+3.41) & 85.37 (+0.20) & 95.38 (+1.29) & 81.43 (+1.29) \\
\midrule
\multicolumn{5}{c}{gemini-pro} \\
\midrule
Plan-and-Solve & 45.68 & 77.15 & 80.74 & 62.29 \\
\rowcolor{gray!25} + Prompt & 47.19 (+1.52) & 78.95 (+1.81) & 80.82 (+0.08) & 63.81 (+1.52) \\
Plan-and-Solve+ & 48.33 & 78.31 & 80.52 & 63.05 \\
\rowcolor{gray!25} + Prompt & 50.11 (+1.78) & 81.97 (+3.66) & 80.74 (+0.23) & 66.19 (+3.14) \\
Zero-Shot CoT & 49.32 & 75.24 & 83.70 & 62.97 \\
\rowcolor{gray!25} + Prompt & 53.87 (+4.55) & 82.13 (+6.89) & 83.70 (+0.00) & 68.74 (+5.77) \\
\midrule
\multicolumn{5}{c}{gpt-3.5-turbo-0125} \\
\midrule
Plan-and-Solve & 42.23 & 81.12 & 78.70 & 63.84 \\
\rowcolor{gray!25} + Prompt & 42.76 (+0.53) & 81.09 (-0.03) & 79.38 (+0.68) & 64.37 (+0.53) \\
\rowcolor{gray!25} + SC & 60.50 (+18.27) & 84.15 (+3.03) & 87.04 (+8.34) & 73.24 (+9.40) \\
Plan-and-Solve+ & 47.54 & 80.55 & 80.67 & 64.97 \\
\rowcolor{gray!25} + Prompt & 49.96 (+2.43) & 81.50 (+0.95) & 81.96 (+1.29) & 66.79 (+1.82) \\
\rowcolor{gray!25} + SC & 60.73 (+13.19) & 83.71 (+3.16) & 87.79 (+7.13) & 73.49 (+8.51) \\
Zero-Shot CoT & 47.69 & 79.94 & 80.89 & 64.67 \\
\rowcolor{gray!25} + Prompt & 51.93 (+4.25) & 83.55 (+3.60) & 83.40 (+2.50) & 69.67 (+5.00) \\
\rowcolor{gray!25} + SC & 59.89 (+12.20) & 83.07 (+3.13) & 87.34 (+6.44) & 72.55 (+7.88) \\
\midrule
\multicolumn{5}{c}{gpt-3.5-turbo-instruct} \\
\midrule
Plan-and-Solve & 25.32 & 69.98 & 70.20 & 49.13 \\
\rowcolor{gray!25} + Prompt & 23.28 (-2.05) & 70.72 (+0.75) & 69.14 (-1.06) & 48.90 (-0.23) \\
\rowcolor{gray!25} + SC & 41.39 (+16.07) & 70.95 (+0.97) & 80.89 (+10.69) & 57.39 (+8.26) \\
Plan-and-Solve+ & 30.93 & 72.32 & 72.86 & 52.69 \\
\rowcolor{gray!25} + Prompt & 29.95 (-0.99) & 80.19 (+7.87) & 70.05 (-2.81) & 56.18 (+3.49) \\
\rowcolor{gray!25} + SC & 45.56 (+14.63) & 74.20 (+1.88) & 82.56 (+9.70) & 61.26 (+8.57) \\
Zero-Shot CoT & 31.92 & 71.81 & 74.75 & 53.68 \\
\rowcolor{gray!25} + Prompt & 35.10 (+3.18) & 79.94 (+8.13) & 73.69 (-1.06) & 58.91 (+5.23) \\
\rowcolor{gray!25} + SC & 45.41 (+13.50) & 74.98 (+3.17) & 82.71 (+7.96) & 62.02 (+8.34) \\
\bottomrule
\end{tabular}
\caption{Representative results of proprietary LLMs on {\benchmark}.}
\label{tab: main_prompt_result}
\end{table*}

We compare the performance of different proprietary LLMs with varied zero-shot prompting techniques on {\benchmark}. Full experimental results could be obtained from Table \ref{tabapp: full_prompting_results} in Appendix \ref{app: prompting_rslt}, and we extract some representative results in Table \ref{tab: main_prompt_result}. From Table \ref{tab: main_prompt_result} we can obtain following conclusions:

First, \textbf{the accuracy of all LLMs on {\benchmark} degrades with the expansion round arises}. The solving accuracy of LLMs with varied prompting methods on $Q_0$ outperforms that on $Q_4$ over $17.57\%$ on average, which demonstrates that the math reasoning ability of LLMs are heavily hindered by long textual context.

Second, \textbf{LLMs with stronger capability are less impacted by the long textual context than those with insufficient language proficiency.}
% example, GPT-4 and GPT-3.5-instruct
{\metricr} indicates the rate at which the accuracies of LLMs decrease as the number of extension rounds (\textit{r}) increases, and LLMs with higher {\metricr} are less influenced by the extended textual context. From Table \ref{tab: main_prompt_result}, we can observe that the {\metricr} of \texttt{Claude-3-opus} on all of three prompting techniques are larger that $83\%$, while the {\metricr} of \texttt{gemini-pro} and \texttt{GPT-3.5-turbo} are mostly lower than $80\%$, indicating that the math reasoning ability of these LLMs with weak language capability is more vulnerable to long contexts.

% Fourth, different prompt techniques could lead to diverse behaviors of LLMs. For \texttt{Gemini-Pro} and \texttt{GPT-3.5-turbo}, \textbf{Zero-shot CoT} can offer greater performance on $R_0$, but also bring quicker accuracy degradation as extension round increases, consequently resulting in limited robustness. Reversely, 



\subsection{RQ2: Improving {\property} by Prompting}\label{sec: rslt-newprompt}
Based on the existing prompting methods, we devise an elaborate prompt inspired by cognitive theory \cite{CLT1998sweller} and incorporate Self-Consistency to attempt to further enhance the capability of LLMs to solve long context math problems. From Table \ref{tab: main_prompt_result}, we can draw following observations.

First,\textbf{ with the help of our newly proposed prompt, enhancements are observed in the performance of most LLMs on the {\benchmark}}, particularly evident in higher rounds of the {\benchmark}.
The experimental result, 
% examples
on one hand, indicates the correctness of our hypothesis that the performance degradations of LLMs may caused by struggling to summarize the given conditions and ultimate objective of long context math problems,
on the other hand, demonstrates the efficacy of our approach for solving long context math problems, attempting to extract useful given conditions, final goal and disregard the unimportant information firstly, then conduct sophisticated math reasoning based on the carefully extracted information to solve the problem.

Second, Self-Consistency (SC) could comprehensively enhance the math reasoning ability of LLMs. With SC, not only the solving accuracy on each round of {\benchmark}, but {\metrice} and {\metricr} are also bolstered, strengthening their reasoning ability and robustness to math problems with long context simultaneously.

Despite above prompting methods could comprehensively alleviate the long context issue of LLMs, there still exists a significant disparity persists between the accuracy on $Q_0$ and $Q_R$, which depicts that long context math problems present additional challenges to LLMs that that our prompt to emphasize given conditions or SC to clarify ambiguities cannot fully overcome.



\subsection{RQ3: SFT Results}\label{sec: rslt-sft}

Representative results are summarized in Table~\ref{tab: sft_rslt} with additional experimental outputs for more LLMs with varying model sizes and backbones shown in Table~\ref{tabapp: sft_full_results} in Appendix~\ref{app: sft_rslt}.
Analysis of Table~\ref{tab: sft_rslt} yields several critical observations.


Firstly, \textbf{SFT on {\sftdata} consistently and significantly enhances {\property} across a range of mainstream open-source LLMs}, as reflected in metrics {\metrice} and {\metricr}. 
On average, SFT on $D$ leads to an improvement exceeding $27\%$  in {\metrice} and over $13\%$ in {\metricr}.
In particular, for Mistral-7B, there is a substantial absolute enhancement of $35.49\%$ in {\metrice} and $21.99\%$ in {\metricr} post-SFT. 
This indicates that fine-tuned LLMs demonstrate heightened effectiveness in solving math word problems with lengthy contexts and exhibit increased resilience against performance degradation in such a scenario.


\begin{table}[ht]
\centering
\footnotesize
\begin{tabular}{ccc}
\toprule
\thead{Model} & \thead{CoLeG-E} & \thead{CoLeG-R}\\
 \midrule
 \multicolumn{3}{c}{Open-source General Pre-trained LLMs} \\
 \midrule
LLaMA-2-7B & 4.31 & 66.71 \\
\rowcolor{gray!25}
 + SFT on D & {28.09  (+23.78)} & {80.97  (+14.26)} \\
 \hline
 LLaMA-2-13B & 8.61 & 70.18 \\
\rowcolor{gray!25}
 + SFT on D & {37.27  (+28.66)} & {\textbf{84.78}  (+14.60)} \\
 \hline
 Mistral-7B & 13.01 & 61.66 \\
\rowcolor{gray!25}
 + SFT on D & {48.50 (+35.49)} & {83.65  (+21.99)}\\
 \hline
 LLaMA-2-70B & 26.50 & 81.19 \\
\rowcolor{gray!25}
 + SFT on D & {\textbf{49.81}  (+23.31)} & {84.57  (+3.38)} \\
 \midrule
 \multicolumn{3}{c}{Specialized Mathematical LLMs} \\
 \midrule
 deepseek-math-7b & 42.98 & 69.07 \\
\rowcolor{gray!25}
 + SFT on D & {51.31  (+8.33)} & {80.34  (+11.27)} \\
 \hline
 WizardMath-70B & 45.97 & 78.75 \\
\rowcolor{gray!25}
 + SFT on D & {54.68  (+8.71)} & {82.60  (+3.85)} \\
  \hline
 MAmmoTH-70B & 42.98 & 85.24 \\
\rowcolor{gray!25}
 + SFT on D & {55.15  (+12.17)} & {83.25  (-1.99)} \\
  \hline
 MetaMath-70B & 52.81 & 80.86 \\
\rowcolor{gray!25}
 + SFT on D & {\textbf{57.12}  (+4.31)} & {\textbf{84.55 } (+3.69)} \\
\bottomrule
\end{tabular}
\caption{Results of the effect of SFT on {\property}. 
All figures are in $\%$, and the SFT results are shaded. 
Differences between SFT results and the original ones are included in parentheses.
The best {\metrice} and {\metricr} are shown in bold.}
\label{tab: sft_rslt}
\end{table}


Secondly, \textbf{employing a more powerful backbone model enhances both effectiveness and robustness, observable before and after SFT on {\sftdata}.}
Among all general pre-trained LLMs evaluated, LLaMA-2-70B demonstrates superior performance, achieving the highest {\metrice} and {\metricr}, both before and after SFT.


Thirdly, \textbf{SFT on {\sftdata} can also facilitate specialized mathematical LLMs in terms of {\property}.}
Various specialized LLMs, such as MetaMath \citep{metamath2023yu}, have been adapted from generally pre-trained models to focus on the mathematical domain.
These LLMs have typically undergone training with extensive CoT data related to GSM8K, making them more effective and robust in solving complex mathematical questions. 
Remarkably, applying SFT on {\sftdata} can further improve their {\property}, as shown in Table~\ref{tab: sft_rslt}.


To delve deeper into the impact of SFT on {\property}, we analyze the accuracy across different rounds of extended problems ($\text{Acc}_I$) in the {\benchmark} dataset.
Our focus encompasses the LLaMA-2 family for general pre-trained LLMs and MetaMath for specialized LLMs, with model sizes spanning 7B, 13B, to 70B. 
As illustrated in Figure~\ref{fig: breakup}, \textbf{there is a noticeable trend of diminishing accuracy from one round to the next for all LLMs, both prior to and after SFT.}
This trend highlights the increased difficulty in solving longer questions, a challenge that mirrors the human experience (Section~\ref{sec: statistical test}).
Importantly, SFT on {\sftdata} yields a substantial accuracy enhancement across all rounds for both LLaMA-2 and MetaMath models. 
Moreover, \textbf{the rate of accuracy decline from round to round is mitigated post-SFT.}


Interestingly, the accuracy of post-SFT LLaMA-2 can be comparable to or even exceed pre-SFT MetaMath, despite the fact that our {\sftdata} consists of only around 65K CoT data compared to 400K that MetaMath has been trained on.
This observation suggests that \textbf{expanding the questions included in the training set could serve as an effective data augmentation strategy to improve the mathematical reasoning abilities of LLMs}.





\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{Figures/breakup.pdf}
    \caption{Analysis of $\text{Acc}_i$ varying over rounds in {\benchmark} with LLaMA-2 and MetaMath families with and without SFT on {\sftdata}.
    Left: LLaMA-2-7B and MetaMath-7B; middle: LLaMA-2-13B and MetaMath-13B; right: LLaMA-2-70B and MetaMath-70B. 
    "w" and "w/o" stand for "with" and "without" respectively.}
    \label{fig: breakup}
\end{figure*}



Our SFT data includes only one round of extension $D_1$ (Section~\ref{sec: exp-sft}), we propose the potential for further extensions of $D_1$ using methods described in Section~\ref{sec: dataset creation} to get $D_2$.
After quality control, $D_2$ encompasses 24,147 valid CoT data (Section~\ref{app: sft_example}).
To examine the effect of scaling up SFT data on {\property}, we analyze four distinct configurations with the LLaMA-2 model family: without SFT, SFT on $D_0$, SFT n $D_0, D_1$, SFT on $D_0, D_1, D_2$.


Figure~\ref{fig: scaleup-e} shows {\metrice} in different SFT settings and model sizes.
The results reveal that, regardless of model size, applying SFT to the answer-augmented GSM8K dataset significantly outperforms the baseline without SFT.
Moreover, \textbf{including extended questions ($D_1$) significantly enhances the models' capability to solve intricate math word problems, and further expansion to include $D_2$ slightly increases efficacy}.
These findings underscore the value of integrating problems with extensive context into SFT data.


Figure~\ref{fig: scaleup-acc} provides a detailed analysis of accuracy in each round for the LLaMA-2-7B model under diverse SFT settings.
The outcomes demonstrate that \textbf{incorporating an increasing number of extended questions into the SFT dataset helps to mitigate the accuracy drop from one round to the next}.





\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Figures/scaleup-e.pdf}
    \caption{{\metrice} of scaling up {\sftdata} across various model scales in the LLaMA-2 family. 
    The results suggest scaling up model scales and {\sftdata} can further improve {\property}.}
    \label{fig: scaleup-e}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Figures/scaleup-acc.pdf}
    \caption{The changes in $\text{Acc}_i$ when LLaMA-2-7B is fine-tuned on different {\sftdata} dataset. 
    Scaling up {\sftdata} improves accuracy in all {\benchmark} subsets.}
    \label{fig: scaleup-acc}
\end{figure}

\subsection{RQ4: OOD Generalization}\label{sec: rslt-ood}

To evaluate the efficacy of our proposed prompting techniques and fine-tuned models on GSM-IC benchmark, which is a variation of GSM8K benchmark involving the inclusion of irrelevant context in the problem. 
Following \cite{distractibility2023Shi}, we uniformly sample 4,000 examples from GSM-IC benchmark to form GSM-IC-4K dataset. 
We evaluate the generalization ability of LLMs from two aspects: the performance of proprietary LLMs with various prompting techniques and Open-source LLMs (specifically LLaMA-2-series) with different model scales. 
%For Open-source LLMs, we choose prompt in Table \ref{tabapp: eval_prompt} for evaluation. 
The results are presented in Table \ref{tab: gsm_ic_4k_result_1} and \ref{tab: gsm_ic_4k_result_2} respectively.

From Table \ref{tab: gsm_ic_4k_result_1}, first, we can observe that except for \texttt{GPT-3.5-instruct} with Zero-shot CoT, \textbf{our proposed prompting can also improve the capability of LLMs for handling math problems with irrelevant context}, further demonstrating the reasonability and effectiveness of our prompt. 
Second, \textbf{more proficient LLMs are less affected by irrelevant context.}
On average, \texttt{GPT-3.5-turbo} surpasses \texttt{GPT-3.5-instruct} by 31.15\% across three types of prompting methods, indicating that LLMs with poor language abilities are struggle in distinguishing between misleading information in questions and genuinely effective known conditions for problem-solving.

From Table \ref{tab: gsm_ic_4k_result_2}, we observe that \textbf{applying SFT on {\sftdata} can drastically improve generalization capability across all Open-source LLMs of various scales on the GSM-IC-4K dataset}, with an average improvement of $26.89\%$. 
Moreover, we can notice that the magnitude of improvement diminishes with increasing model scale, showing that the characteristics and tendencies of smaller-scale LLMs are more readily adaptable to the target domains of SFT data.


In general, \textbf{both our proposed prompt methods and the SFT procedure comprehensively enhance the generalization ability of proprietary LLMs and open-source LLMs on GSM-IC-4K dataset}, further demonstrating their rationality and effectiveness.

\begin{table}[ht]
\centering
\footnotesize
\begin{tabular}{ccc}
\toprule
% \thead{Model} & \thead{CoLeG-E} & \thead{CoLeG-R}\\
 & \thead{GPT-3.5-turbo} & \thead{GPT-3.5-instruct} \\ % & \thead{LLaMA-2-70B} & \thead{LLaMA-2-70B-SFT} \\
 \midrule
 % SFT-Prompt & - & - & \textbf{65.70} & 85.22 \\
 % \midrule
 Plan-and-Solve & 85.38 & 50.52 \\% & 55.80 & \textbf{85.25} \\
 \rowcolor{gray!25} +Prompt & \textbf{85.90} & \textbf{52.85} \\% & 53.00 & 79.55 \\
 \midrule
 Plan-and-Solve+ & 87.48 & 51.65 \\% & 57.78 & 82.82 \\
 \rowcolor{gray!25} +Prompt & \textbf{91.63} & \textbf{57.50} \\% & 55.42 & 80.32 \\
 \midrule
 Zero-shot CoT & 88.35 & \textbf{65.60} \\% & 44.15 & 84.38 \\
 \rowcolor{gray!25} +Prompt & \textbf{90.05} & 60.98 \\% & 49.90 & 79.10 \\
\bottomrule
\end{tabular}
\caption{Solving accuracy of proprietary LLMs on GSM-IC-4K. All figures are in \%.}
\label{tab: gsm_ic_4k_result_1}
\end{table}

\begin{table}[ht]
\centering
\footnotesize
\begin{tabular}{cc}
\toprule
% \thead{Model} & \thead{CoLeG-E} & \thead{CoLeG-R}\\
 \thead{Open-source Models} & \thead{Accuracy} \\
 \midrule
 LLaMA-2-7B & 33.55 \\
 \rowcolor{gray!25} +SFT on D & \textbf{66.48} (+32.93) \\
 \midrule
 LLaMA-2-13B & 48.45 \\
 \rowcolor{gray!25} +SFT on D & \textbf{76.68} (+28.23) \\
 \midrule
 LLaMA-2-70B & 65.70 \\
 \rowcolor{gray!25} +SFT on D & \textbf{85.22} (+19.52) \\
\bottomrule
\end{tabular}
\caption{Solving accuracy (in $\%$) of LLaMA-2-series on GSM-IC-4K.}
\label{tab: gsm_ic_4k_result_2}
\end{table}


==> Chapters/gsm8k_lc.tex <==
\section{The {\benchmark} Dataset}





\subsection{LLMs Struggle to Answer Math Wrod Problems with Longer Descriptions}\label{sec: statistical test}

To explore whether the performance of LLMs in mathematical reasoning is adversely affected by longer textual contexts, similar to human performance, we conducted an experiment on GSM8K using CoT with \texttt{GPT-3.5-turbo}. 
The experiment employed the 8-shot demonstrations provided by \citet{CoT2022Wei}, and the complete prompt can be found in Appendix~\ref{app:prompt}.
We can compare the answers generated by LLMs with the ground-truth answers and then divide the examples into two groups based on accuracy: the correct answers group $G_0$ and the incorrect answers group $G_1$. 

We want to study whether there exists a significant difference in the length of problem descriptions, characterized by the number of tokens, between these two categories.
We hypothesized that the lengths of the problem descriptions of these groups are drawn from different distributions, denoted $X$ and $Y$.
The one-sided Mann-Whitney test \citep{MWtest1947Mann} is applied:
\begin{equation*}
    \begin{aligned}
        H_0:\ P(X<Y) &= P(X>Y)  \\
        \leftrightarrow H_1:&\ P(X<Y) > P(X>Y)
    \end{aligned}
\end{equation*}


The results are reported following \citet{MWtestExplain2012Fritz}: There is significant evidence indicating that the number of tokens in $G_0$ is less than in $G_1$ with $U=141565, P = 0.0000$. 
This finding strongly suggests that, akin to humans, LLMs exhibit reduced performance on math word problems with longer textual contexts.




\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Figures/acc_tokens.pdf}
    \caption{Boxplot illustrating the distribution of "the number of tokens" across two distinct groups delineated by True and False in their answers.
    The visual comparison suggests the number of tokens in the False group is larger than the True group, with the Mann-Whitney U test providing evidence regarding the significance of these differences.
    This implies that LLMs struggle to do math reasoning in math word problems with longer context, which is similar to humans.}
    \label{fig: acc_tokens}
\end{figure}




\subsection{Dataset Creation}\label{sec: dataset creation}


\begin{table}
    \footnotesize
    \centering
    \begin{tabular}{l|ccccc}
        \toprule
        Round &$Q_0$ & $Q_1$ & $Q_2$ & $Q_3$ & $Q_4$\\
        \midrule
        \#Tokens &77.0 & 192.2 & 301.5 & 363.5 & 385.7 \\
        \hline
        \#Questions& 1319 & 1195 & 1143 & 1102 & 1068\\
        \bottomrule
    \end{tabular}
    \caption{The average tokens of {\benchmark} dataset where the number of tokens is returned by GPT-4-turbo and the number of questions in each round of extension.}
    \label{tab:tokens}
\end{table}

To conduct a more nuanced analysis of {\property} across a range of LLMs, we have created {\benchmark} as a testing ground.
This section will detail the construction process.


Our approach leverages \texttt{GPT-4-turbo} to expand the original set of problems from GSM8K.
Initial trails revealed that the augmented questions were only slightly longer than their original questions, and \texttt{GPT-4-turbo} failed to achieve a specified token length as set out in the instructions.
To overcome this issue and facicitate the extension of math problems into more elaborate contexts, we adopted a sequential, iterative strategy.
During the $r$-th iteration, each question from the preceding iteration $(r-1)$, denoted as $q_{r-1} \in Q_{r-1}$, is extended using 2-shot demonstrations with \texttt{GPT-4-turbo}.
Following the expansion in the $r$-th round, a meticulous filtering step is performed to ensure quality (see Appendix~\ref{app:human eval}), resulting in the refined set of expanded problems, $Q_r$.
The prompt structure, along with the entire extension process, is depicted in Figure~\ref{fig:extension_illustration}.
It is crucial to note that our prompt instructions require that the extension preserve the integrity of the original problem, including its inherent meaning, sequence of presentation, and the ground-truth answer.
Human evaluation is also conducted to ensure these aspects.


The process commences with the GSM8K \citep{gsm8k2021cobbe} test set  used by \citet{zero-shot-CoT2022Kojima}\footnote{The test set can be accessed through \href{https://github.com/kojima-takeshi188/zero_shot_cot/blob/main/dataset/grade-school-math/test.jsonl}{this link}}.
This iterative procedure ends after the completion of the $R$-th round of expansion, where $R=4$ for our purposes.
The full prompts can be found in Appendix~\ref{app:prompt}.


As each round of expansion progresses, we observe a gradual increase in the length of the questions. 
The average token count for the mathematical problems in each stage is presented in Table~\ref{tab:tokens}.
In the later phases of our extension process, a deceleration in the rate of increase in the number of tokens is observed, leading us to end the expansion at $R=4$.
As a result, our {\benchmark} incorporates the extended problems from all rounds (subject to quality control) $\cup_{r=1}^R Q_r$.
Some examples are provided in Appendix~\ref{app:statistics}.


Human evaluation is carried out to ensure the quality of {\benchmark}.
50 seed questions are selected from GSM8K and all questions derived from these selected questions are manually inspected.
These questions are categorized into three quality levels.
\begin{itemize}
    \item \textbf{Excellent}. The ground-truth answer and conditions of the extended problem are the same as in the original problem.

    \item \textbf{Good}. The ground-truth answer of the extended problem is not changed. However, the conditions of the extended problem are vague. As a result, there may be multiple interpretations of these extended problems.

    \item \textbf{Poor}. The ground truth answer or the conditions of the problems were changed during the extension process.
\end{itemize}
Appendix~\ref{app:human eval} provides several examples for each quality level. 
Our evaluation finds that 185 of the 200 extended problems (50 seed problems x 4 rounds) are of excellent quality, 4 are good and 11 are poor. 


To economize human effort, we apply the following heuristics to automatically filter out our undesired examples.
For each seed question $q_0^i$ and its associated extended variants $q_1^j, ... ,q_R^j$, we derive a score $S_r^i = ENT(q_r^i, q_0^i)$ to evaluate the informational equivalence between the extended and the seed questions.
More specifically, we adopt the out-of-box entailment model \citep{summac2022laban} to calculate $S_r^i$ (see Appendix~\ref{app: ent}).
A small $S_r^i$ can suggest a potentially unsatisfactory extension, leading to the exclusion of the question $q_r^i$ if $S_r^j < 0.2, \text{for any} j \leq r$.
Obviously, $Q_{r} \subseteq Q_{r-1}$ after filtration.
Through this quality control heuristic, we successfully filter out examples under good and poor quality levels. 
The number of questions retained in each round is shown in Table~\ref{tab:tokens}.

%To ensure the quality of the dataset, specifically to ensure that the answers to the problems, the problem conditions, and the order of the conditions remain consistent, we performed a human evaluation. During the human evaluation process, we randomly selected 50 samples from each round of the expanded dataset. We then reviewed a total of 200 samples to identify any instances where the ground truth answer or conditions of the problems were changed during the expansion process, and called these extended problems "extend false"

%Through human evaluation, we found that 11 out of 200 extended problems are "extend false". These problems had their conditions changed during the expansion process. Afterwards, we used the ent-based method to filter out questions with an ent score of less than 0.2. We found that this method successfully identified the samples where the questions were extended incorrectly among the 50 identified IDs. As a result, we obtained a higher quality dataset that was more suitable for use in our experiment.






\subsection{Evaluation Metrics}\label{sec: evaluation}


For a given question $q$, its ground-truth answer is denoted by $gt(q)$, and the answer generated by the method {\method} is represented as {\method}$(q)$.
Inspired by \citet{distractibility2023Shi}, the following metrics are considered to assess the performance of {\method} on math word problems with extended context:

\textbf{Round-$r$ accuracy} $\text{Acc}_r(\mathcal{M})$ = $Acc(\mathcal{M}; Q_r)$ is defined as the average accuracy of method {\method} on the set of problems $Q_r$.

\begin{equation*}
\text{Acc}(\mathcal{M}; Q_r) =\frac{\sum_{q \in Q_r} \mathbb{I}[\mathcal{M}(q)=gt(q)]}{|Q_r|},
\end{equation*}
where $|\cdot|$ denotes the number of questions in a set.

\textbf{\metrice} quantifies the \textbf{e}fficacy of \textbf{{\property}}, which is defined as the averaged accuracy of {\method} to solve a seed question and all its corresponding extension variants.
\begin{equation*}
    \text{\metrice} (\mathcal{M}) = \frac{\sum_{q_R^i \in Q_R} \left[ \wedge_{r = 1}^R \mathbb{1}[\mathcal{M}(q_r^i)=gt(q_r^i)] \right] }{|Q_R|},
\end{equation*}
indicating that {\metrice} evaluates the proportion of original problems that can be consistently solved across all levels of extended context.

\textbf{\metricr} assesses the \textbf{r}obustness facet of \textbf{{\property}}, which is characterized by the relative accuracy drop rate on $Q_R$ compared to the performance on initial questions $Q_0$:
\begin{equation*}
    \text{\metricr} (\mathcal{M}) = 1- \frac{\text{Acc}_0(\mathcal{M}) - \text{Acc}_R(\mathcal{M})}{\text{Acc}_0(\mathcal{M})}.
\end{equation*}

%\textbf{Total accuracy} $Acc_{all}(\mathcal{M})$ represents the mean accuracy of {\method} across classes of test problems, where each class $Q(b)$ includes test questions extended from the same original question $b \in Q_0$. 
%The method {\method} is defined to correct on a class $Q(b)$ if and only if it accurately resolves all %problems within this class.

%\begin{equation*}
%Acc_{all}(\mathcal{M}) =\frac{\sum_{q \in Q_0} \left[ \wedge_{q \in Q(b)} \mathbb{1}[\mathcal{M}(q)=gt(q)] \right] }{|Q_0|},
%\end{equation*}
%indicating that total accuracy evaluates the proportion of original problems that can be consistently solved across all levels of extended context.


%\textbf{Normalized accuracy} $Acc_{norm}(\mathcal{M})$ quantifies the impact of extended contexts on the performance of {\method}, relative to its accuracy in original questions:
%\begin{equation*}
%Acc_{norm}(\mathcal{M}) = \frac{Acc_{all}(\mathcal{M})}{Acc(\mathcal{M}; Q_0)}.
%\end{equation*}


==> Chapters/intro.tex <==
\section{Introduction}


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Figures/extension_process.pdf}
    \caption{{\benchmark} Creation Process and Prompt Template for Extension.
    \texttt{GPT-4-turbo} is prompted to iteratively extend the original math word problems into ones with longer and longer descriptions.}
    \label{fig:extension_illustration}
\end{figure}

Math word problems \citep{MWP1964bobrow} are mathematical questions presented in natural language, demanding mathematical reasoning for solving.
The advent of large language models (LLMs) \citep{GPT32020Brown, mixtral-8x7b2024Albert, Llama2023Touvron, GPT42023openai} has spurred the development of various prompting techniques to improve mathematical capabilities \citep{CoT2022Wei, zero-shot-CoT2022Kojima, Plan-Solve2023Wang, selfdiscover2024Zhou}. 
Typically, these methods are often tested on benchmarks such as GSM8K \citep{gsm8k2021cobbe}, characterized by problem descriptions that consist of a few concise sentences.
However, this setting differs from real-world scenarios, where contexts can be complex and lengthy. 
Research in educational theory \citep{mathcontext1993Boaler} suggests that complex or extensive contexts might hinder rather than facilitate the mathematical reasoning process.
This observation leads to a pertinent question: Do LLMs exhibit a similar phenomenon?


To explore this phenomenon, the chain-of-thought \citep{CoT2022Wei} (CoT) is conducted on GSM8K and segregating the questions based on the accuracy of the CoT predictions. 
Rigid statistical hypothesis testing has revealed significant evidence suggesting that LLMs exhibit decreased performance on the question with longer problem descriptions (Section~\ref{sec: statistical test}).
This study is dedicated to examining the \textbf{Co}ntext \textbf{Le}ngth \textbf{G}eneralizability (\textbf{{\property}}) of LLMs in math reasoning, with a specific focus on the following research questions:

RQ1. How are different LLMs and prompting techniques affected by lengthy contexts in mathematical reasoning? (Section~\ref{sec: exp-prompting} and \ref{sec: rslt-prompting})

RQ2. How could we potentially improve {\property} of LLMs by prompting? (Section~\ref{sec: exp-newprompt} and \ref{sec: rslt-newprompt})

RQ3. To what extent can Supervised Fine-Tuing (SFT) enhance {\property}? (Section~\ref{sec: exp-sft} and \ref{sec: rslt-sft})

RQ4. How effective are our novel prompting techniques and fine-tuned models when applied to other variants of the math word problem benchmark like GSM8K-IC \citep{distractibility2023Shi}? (Section~\ref{sec: rslt-ood})
%and R-GSM \citep{premiseorder2024chen}? (Section~\ref{sec: rslt-ood})



To investigate these research questions, we construct the {\benchmark} dataset (Figure~\ref{fig:extension_illustration} and Section~\ref{sec: dataset creation}), comprising math word problems with extended contexts derived from GSM8K. We also introduce metrics to evaluate the efficacy and robustness of LLMs in handling these problems (Section~\ref{sec: evaluation}). 
Unlike existing works that generate benchmark variations through automated perturbations, our approach emphasizes minimal alterations to the original problem conditions and the description order. 
This approach ensures the preservation of the original ground-truth answers, as confirmed through human evaluation (see Section~\ref{sec: dataset creation} and Appendix~\ref{app:human eval}).

To address RQ1, we have assessed the perofrmance of [how many] proprietary LLMs, together with three state-of-the-art zero-shot prompting techniques on {\benchmark}, including 0-CoT \citep{zero-shot-CoT2022Kojima}, PS \citep{Plan-Solve2023Wang}, and Self-Discover \citep{selfdiscover2024Zhou}. 
Our findings indicate that {\property} of these prompting approaches are somewhat limited, urging further exploration of strategies to alleviate this problem (RQ2). 
As part of our mitigation efforts, we introduce task-specific instructions and investigate self-consistency (SC) \citep{CoT-SC2022Wang}. 
Beyond prompting strategies, we also explore SFT as a way to enhance {\property} of LLMs.
This investigation includes applying SFT to 18 open-source LLMs across model scales and task-specific fine-tuning strategies.

We summarize our key findings below:

1. Across all zero-shot prompting examined, we observed a decrease in accuracy in {\benchmark} among closed-source LLMs with each additional round of expansion. Notably, LLMs with higher initial proficiency exhibited a diminished susceptibility to the challenges posed by extended contexts.

2. The implementation of our instructional prompt strategy leads to an enhancement in the {\property} of LLMs. Incorporating self-consistency further augments these improvements.

3. Applying SFT with our newly introduced {\sftdata} dataset notably increases the {\property} of LLMs. Furthermore, enhancements are more pronounced when scaling up the application of {\sftdata}.

4. Our innovative prompting technique and the fine-tuned LLMs demonstrate their efficacy on GSM-IC.


Extracting information from a lengthy context to perform mathematical reasoning is essential for real-world tasks.
Our work pioneers the assessment of {\property}, and our new prompting methods and SFT methods will not degrade the performance of original mathematical reasoning, while improving {\property} of LLMs substantially.
Additionally, our findings suggest another possible boostrapping \citep{metamath2023yu} method to augment the training set.
Our study suggests a path forward: To achieve a comprehensive understanding of the reasoning capabilities of LLMs, future research should also pay attention to evaluating the models' efficacy and resilience in solving math word problems with extensive contexts.




==> Chapters/limitation.tex <==
\section*{Limitations}








\section*{Ethics Statement}

==> Chapters/method.tex <==
\section{Experimental Setup}
In this section, we decribe the LLMs used to investigate {\property} (Section~\ref{sec: exp-llms}), the evaluated prompting techniques (Section~\ref{sec: exp-prompting}), strategies for enhancing {\property} through prompting (Section~\ref{sec: exp-newprompt}), and experimental setup for SFT (Section~\ref{sec: exp-sft}). 
To report the results, we use \texttt{GPT-3.5-turbo} to extract the final answers in case that responses may not follow the desired format. 
Human evluation shows that our answer extraction methods successfully get the final answer [what percentage] and details are provided in Appendix~\ref{app: answer_ext}.


\subsection{Investigated LLMs}\label{sec: exp-llms}

Our investigation of various prompting techniques (Section~\ref{sec: exp-prompting} and \ref{sec: exp-newprompt}) leverages a variety of closed-source LLMs.
We include comprehensive mainstream proprietary LLMs such as GPT-4 \citep{GPT42023openai}, GPT-3.5-turbo, GPT-3.5-instruct, Gemini-pro \citep{gemini2023team}, Claude-3 and mistral-medium. 
For SFT, our study encompasses LLaMA-2 \citep{Llama22023Touvron} across different model scales, Mistral-7B \citep{mistral2023Jiang} and specialized mathematical models, including WizardMath \citep{wizardmath2023luo}, MAmmoTH \citep{mammoth2023yue}, MetaMath \citep{metamath2023yu}, and Llemma \citep{llemma2023azerbayev} varying in base models and model sizes.
We perform greedy decoding with the temperature 0 to ensure reproducibility.
More detailed descriptions of these LLMs can be found in Appendix~\ref{app: llms}.


\subsection{Investigated Prompting Techniques}\label{sec: exp-prompting}

To negate the influence of few-shot demonstrations, we explore zero-shot prompting techniques, including zero-shot CoT (0-CoT) \citep{zero-shot-CoT2022Kojima}, Plan-and-Solve (PS)\citep{Plan-Solve2023Wang}, and Self-Discover (SD) \citep{selfdiscover2024Zhou}. 

\textbf{Zero-shot CoT} \citep{zero-shot-CoT2022Kojima}, a variant of CoT \citep{CoT2022Wei}, prompts the model directly with the problem of interest followed by "Let's think step by step," without providing any demonstration examples.

\textbf{Plan-and-Solve} \citep{Plan-Solve2023Wang} enhances 0-CoT by initially prompting LLMs to create a plan that breaks down the overarching task into subtasks, subsequently executing these subtasks in accordance with the devised plan. Additionally, we investigate a variant of PS, identified as PS+, designed to mitigate calculation inaccuracies.

\textbf{Self-Discover} \citep{selfdiscover2024Zhou} developed more recently, encourages LLMs to uncover intrinsic task-related reasoning structures to address complex reasoning challenges. This approach involves composing a coherent reasoning structure by selecting relevant modules, tailoring to specific task descriptions, and implementing a reasoning structure in JSON format.


The specific designs for these zero-shot prompts are detailed in [where], and the outcomes are presented in Section~\ref{sec: rslt-prompting}.



\subsection{Improve {\property} by Prompting}\label{sec: exp-newprompt}


In addition to existing prompting methods, we also explore the potential benefits of incorporating natural language instructions to enhance LLMs' {\property}.
Drawing inspiration from cognitive load theory \citep{CLT1998sweller}, which suggests that segmenting extensive information into smaller chunks can facilitate the learning process of students, we devised an instructional prompt. 
This prompt strategy begins by guiding LLMs to identify the conditions and ultimate objective from the given context and then encourages solving the problem step by step.
The structure of this prompt is detailed in [where].
We observed that conventional prompting methods often struggle to accurately extract the relevant conditions from extensive contexts.
Our newly proposed prompt can relieve this issue by ensuring a more efficient comprehension and processing of the given information (see Section~\ref{sec: rslt-newprompt}).


Additionally, we explore the role of self-consistency (SC) \citep{CoT-SC2022Wang} in improving {\property} of LLMs. 
SC operates by generating multiple reasoning paths, followed by aggregating these responses through a majority vote to determine the final answer.
It is important to note that SC is orthogonal to the aforementioned prompting strategies, meaning that it can be integrated with any of them.
For our implementation, we generate 5 responses using a sampling temperature of $0.7$.


\subsection{SFT Setup}\label{sec: exp-sft}

Beyond examining various prompting strategies, we also investigated the effect of integrating longer questions into SFT on {\property} of LLMs. 


To augment our training dataset beyond the 7,473 annotated examples available in GSM8K, we employ CoT data augmentation \citep{metamath2023yu}. 
We generate five reasoning paths for each question in the training set with \texttt{GPT-3.5-turbo} and remove any paths that led to incorrect final answers.
This process yields 38,507 valid CoT data points, denoted by $D_0$.
For the extended questions, we initially expand the questions in the training set through one extension iteration with GPT-4-turbo and quality control with our heuristic (see Section~\ref{sec: dataset creation}) before applying CoT augmentation, resulting in 26,422 CoT data for extended quesitons, denoted by as $D_1$.
The entire training set, represented as $D=D_0 \cup D_1$, incorporates 64,929 CoT data.
Appendix~\ref{app: sft_example} shows the input-output formats of the SFT data and examples from both $D_0$ and $D_1$.


Multiple open-source LLMs, differing in scale and base models as detailed in Section~\ref{sec: exp-llms}, are fine-tuned on $D$.
The fine-tuning is carried out over 3 epochs and the results are reported using 0-CoT with the vLLM library\footnote{\href{https://github.com/vllm-project/vllm}{https://github.com/vllm-project/vllm}.}.
All evaluations adhere to the same 0-CoT instruction set to ensure consistency.
To account for the potential influence of random variations during the training process, we include the performance trends throughout the entire training period in Appendix~\ref{app: training_curves}.
Furthermore, comprehensive details regarding the training and inference parameters can be found in Appendix~\ref{app: sft_detail}.







==> Chapters/related_work.tex <==
\section{Related Work}

\subsection{Prompting for Mathematical Reasoning}

Mathematical reasoning \citep{MWP1964bobrow, gsm8k2021cobbe, MATH2021hendrycks} is recognized as a system-2 task \citep{system22011kahneman, system22021bengio}, attracting significant attention in the research community. 
Recent advancements in LLMs \citep{GPT32020Brown, GPT42023openai, InstructGPT2022Ouyang, mixtral-8x7b2024Albert} have spurred the development of various prompting methods to facilitate mathematical reasoning using LLMs \citep{llm4math2024Ahn}.
Among these, the Chain-of-Thought (CoT) prompting \citep{CoT2022Wei} enhances the reasoning ability of LLMs by incorporating intermediate stepsleading up to the final answers.
Additionally, several few-shot prompting techniques, such as Re-reading \citep{rereading2023xu}, Stepback prompting \citep{Stepback2023Zheng}, PHP \citep{PHP2023Zheng}, and CR \citep{CR2023Zhang}, have been developed to further improve the reasoning capabilities of LLMs in solving mathematical problems.

In contrast, a subset of methods has focused on enabling reasoning in a zero-shot manner, thereby bypassing few-shot demonstrations \citep{zero-shot-CoT2022Kojima, Plan-Solve2023Wang, selfdiscover2024Zhou}.
Specifically, \citet{zero-shot-CoT2022Kojima} introduce a two-stage CoT prompting approach that encourages LLMs to induce reasoning steps using "Let's think step by step". 
Plan-and-Solve (PS) prompting \citep{Plan-Solve2023Wang} further amplifies zero-shot reasoning by formulating a strategic plan prior to tackling mathematical queries. 
Moreover, \citet{selfdiscover2024Zhou} propose a general framework designed to autonomously uncover the task-specific reasoning architectures inherent to LLMs.

Extensions to CoT encompass few-shot demonstration selection \citep{Auto-CoT2022zhang, activeprompt2023Diao, Complexity-CoT2022fu}, advancements in decoding \citep{CoT-SC2022Wang, CoT-decoding2024Wang}, and developments catering to more intricate tasks \citep{react2022Yao, ToT2023Yao, GoT2023Besta, XoT2023Ding}. 
Further explorations within this domain have probed areas such as incorrect answer detection \citep{cot-detection2024xu}, the impact of reasoning length \citep{reasoninglength2024jin}, and investigations of failure modes \citep{reversalcurse2023Berglund, distractibility2023Shi, premiseorder2024chen, gsm-plus2024Li}. 


Our work pioneers the investigation of LLMs' {\property} in mathematical reasoning, employing a zero-shot prompting to isolate the influence of few-shot demonstrations.




\subsection{Specialized LLMs for Mathematics}


With the development of general-purpose LLMs \citep{GPT32020Brown, GPT42023openai, mixtral-8x7b2024Albert, Palm22023anil, Llama2023Touvron, Llama22023Touvron}, there remains a persistent interest in maximizing the performance of LLMs within specific domains, particularly in mathematics. 
These models rely on either supervised fine-tuning or continued pretraining strategies to improve their capabilities.
Several studies have concentrated on supervised fine-tuning using task-relevant input-output pairs. 
For example, WizardMath \citep{wizardmath2023luo} proposes to enhance LLMs by combining supervised fine-tuning with PPO training.
Similarly, MAmmoTH \citep{mammoth2023yue}adopts a knowledge distillation approach by integrating CoT with Program-of-Thought\citep{PoT2022Chen, PAL2023Gao}. 
Additionally, MetaMath \citep{metamath2023yu} rewrites mathematical questions in multiple formats to augment the training dataset.
On the other hand, a distinct strand of research is dedicated to continuing pretraining of base LLMs on extensive mathematical corpora, exemplified by Minerva \citep{minerva202lewkowycz}, Llemma \citep{llemma2023azerbayev}, InternLM-MATH \citep{internlmmath2024ying} and DeepSeekMath \citep{deepseekmath2024shao}.
Our work explores to what extent  {\property} of these specialized mathematical LLMs will be improved by SFT.






==> nips_app/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
%The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
%limit. 

%Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
%\begin{itemize}
%    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
%\end{itemize}

%{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

%The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

%IMPORTANT, please:
%\begin{itemize}
%    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
%\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The main claims made in the abstract and introduction accurately reflect the paper's contributions and scope. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The limitations of the work are discussed in Appendix~\ref{app:limitation} "Limitations". %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNo{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not include theoretical results. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The steps for creating and evaluating our new dataset are presented in Section~\ref{sec: dataset creation} and our new methods are detailed in Section~\ref{sec: our prompt} and \ref{sec: new sft}. All experimental setup and details can be found in Section~\ref{sec: exp_setup} and Appendix~\ref{app: sft_detail}. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our data and code can be found in \href{https://anonymous.4open.science/r/CoLeG-Math-07DE}{https://anonymous.4open.science/r/CoLeG-Math-07DE}.%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The experimental settings are presented in Section \ref{sec: exp_setup} and the details are given in Appendix~\ref{app: sft_detail}. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: It is impractical to run our experiments several times because of our budgets and the computational costs. Following the convention, we use greedy decoding with temperature $0.0$ for reproduction. We also provide statistical significance tests in Section~\ref{sec: statistical test}. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The details of compute resources are discussed in Appendix~\ref{app: sft_detail}. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The authors have reviewed the NeurIPS Code of Ethics and make sure the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The potential positive and negative societal impacts are discussed in Appendix~\ref{app:broader impact} "Broader Impacts". %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper poses no such risks.%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All assets are cited appropriately, and Appendix~\ref{app: llms} and \ref{app: ood_rslt} have provided the licenses and links.%\justificationTODO{}
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our new assets can be found in \href{https://anonymous.4open.science/r/CoLeG-Math-07DE}{https://anonymous.4open.science/r/CoLeG-Math-07DE}. The detailed creation and quality control process are provided in Section~\ref{sec: dataset creation}, \ref{sec:qualitycontrol} and Appendix~\ref{app:statistics}, \ref{app:human eval}, \ref{app: ent}.%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> nips_chapters/limitation.tex <==
\section*{Limitations}\label{app:limitation}

Despite the innovative contributions of newly released {\benchmark}, {\abbrpromptname}, and the \textit{extension} auxiliary task, our work still has some limitations.
1. Data Quality in {\benchmark}: Although heuristic methods are employed to control the quality of {\benchmark}, the dataset may still contain poorly constructed questions. 
Due to budget and time constraints, no complete human review of the dataset was performed. 
A more thorough human evaluation by well-funded institutions would be beneficial.
2. Generalizability Concerns: While the generalizability of our methods has been assessed using GSM-IC, our primary conclusions are derived from variants of the GSM8K dataset.
Including additional benchmarks for MWPs would provide a more robust validation of our findings. 
However, conducting experiments on more datasets is resource-intensive. 
Therefore, we encourage further investigation by the research community.
3. Limited SFT Data: 
Owing to budget limitations, our released SFT data comprises approximately 65K examples. 
Further expansions could involve scaling up the \textit{extension} augmented data, either by increasing the rounds of extension or applying other data augmented techniques.
The exploration of alternative methods to extend SFT data and examining scalability effects also offers interesting avenues for future research.
4. Interpretability and Explainability:
Even with the improved performance achieved by our methods, LLMs remain "black boxes." 
Understanding the intricate reasoning processes behind their solutions continues to be a significant challenge. 
In this study, synthetic data is used to evaluate the impact of long context on the mathematical reasoning
ability of LLMs. It is also used to augment training data to improve model robustness. To mitigate potential
misuse of synthetic data, we have documented the generation process and intended use of synthetic data,
ensuring that any assumptions or limitations are publicly communicated.





\section*{Broader Impacts}\label{app:broader impact}

Our release of {\benchmark} presents a challenging benchmark to test the ability of LLMs to solve long MWPs.
This aids future research by highlighting the intricacies involved in extended MWPs.
Our innovative prompting method and the SFT technique have improved LLMs performance in these problems, potentially enhancing their generalization capabilities for real-world applications.
This advancement not only broadens LLMs' mathematical reasoning capacities, but also has implications for educational tools.
However, despite progress, significant challenges in solving extended MWPs remain, calling for future refinements.
Additionally, there is a risk of overreliance which might impede the development of critical thinking skill and problem-solving skills for human learners.
Therefore, we point out the need for balanced use of LLM technologies, combining their benefits with critical human oversight.





